Beyond PID Controllers: PPO with Neuralized PID Policy for Proton Beam Intensity Control in Mu2e

We introduce a novel Proximal Policy Optimization (PPO) algorithm aimed at addressing the challenge of maintaining a uniform proton beam intensity delivery in the Muon to Electron Conversion Experiment (Mu2e) at Fermi National Accelerator Laboratory (Fermilab). Our primary objective is to regulate the spill process to ensure a consistent intensity profile, with the ultimate goal of creating an automated controller capable of providing real-time feedback and calibration of the Spill Regulation System (SRS) parameters on a millisecond timescale. We treat the Mu2e accelerator system as a Markov Decision Process suitable for Reinforcement Learning (RL), utilizing PPO to reduce bias and enhance training stability. A key innovation in our approach is the integration of a neuralized Proportional-Integral-Derivative (PID) controller into the policy function, resulting in a significant improvement in the Spill Duty Factor (SDF) by 13.6%, surpassing the performance of the current PID controller baseline by an additional 1.6%. This paper presents the preliminary offline results based on a differentiable simulator of the Mu2e accelerator. It paves the groundwork for real-time implementations and applications, representing a crucial step towards automated proton beam intensity control for the Mu2e experiment.

==> boarder.tex <==
To be filled.

==> method_old.tex <==
In this section, we first introduce . Then, we provide a detail design of how we 

\subsection{Problem Setup}

Currently, Fermilab's focus is on its world-class experimental program at the intensity frontier. While increasing beam intensity poses its own challenges, maintaining beam size and minimizing beam losses - particles lost due to interactions with the beam vacuum pipe - are often the primary obstacles. The accelerator is regulated by a sophisticated system comprising hundreds of thousands of devices. 
Employing machine learning methods for fine-tuning and real-time optimization of these parameters, moving beyond the experience-based reasoning of human operators is crucial for the success of future intensity upgrades.

\paragraph{Objective.}
To handle the challenges posed by Mu2e experiment, we need to regulate the uniformity of the extracted spill --- or increase its Spill Duty Factor (SDF), 
\bea
\text{SDF}\coloneqq1/\left({1+\sigma_{\text{spill}}^2}\right),
\text{SDF}\coloneqq1/\left({1+\sigma_{\text{spill}}^2}\right),
\eea
by regulating the extraction process.
The ultimate goal for SRS in the Mu2e experiment is to achieve a SDF of 0.6 or higher, with an ideal spill having a constant spill rate value of 1 and an SDF of 1.The subsequent sections of this paper commence by introducing the Mu2e simulator and outlining the problem setup. We then proceed to provide a detailed description of our proposed method. Subsequently, we present numerical results to showcase the performance of our approach. Finally, we conclude this paper with a discussion of potential future directions and avenues for further research.

\begin{itemize}[leftmargin=*,before=\vspace{-0.3em}, after=\vspace{-0.3em}]
\setlength\itemsep{0em}
    \item 
    \textbf{Existing Approach: PID Controllers}\\
    Proportional-Integral-Derivative controllers (PIDs) are linear, symmetric heuristic control systems with constant parameters. They are designed to operate in domains where the system's response remains \textit{invariant} across all operating regions. 
    Although PID controllers are relatively robust and well-established, they struggle to manage the non-linearity of the resonance process, short spill durations, and the stringent requirements for spill quality imposed by the Mu2e experiment.
    \item 
    \textbf{Proposed Approach: Learned Controllers}\\
    Moreover, since we cannot assume the precise noise distribution and potential non-linearities in the extraction system, a control system capable of adapting to the extraction system's nonlinearities is necessary. 
    To this end, we propose using RL-enhanced learned controllers.
\end{itemize}

\subsection{PPO Controller}




\paragraph{Reward Function.}
In this work, we focus on the tracking problem, in which there are a set of signals (spill intensity) that we wish to maintain at given reference values (close to 1).
Let $x_t$ be the observation of one single spill signal at time step $t$ and $\sigma = 1$ be the corresponding reference value, respectively.
The reward function at $t$ is defined as the exponential moving average
\bea
r_t=-{\rm EMA}(t,\alpha), 
\eea
where
\bea
{\rm EMA}(t,\alpha) = \alpha|x_t - \sigma| + (1-\alpha){\rm EMA}(t-1,\alpha),
\eea
and $\alpha \in \[0, 1\]$. 
EMA gives more weight to recent spills and less weight to older spills. This helps in reducing the impact of short-term fluctuations in the spills, making it easier to identify underlying trends or patterns.

\paragraph{PID Inductive Bias.}
PID controller encodes historical information about tracking errors, integrals of tracking errors, and derivatives of tracking errors in a linear policy framework. 
Formally, the policy of the discrete-time PID controller, with its parameter $K_P$, $K_I$, and $K_D$, is given as
\bea
\pi^{\text{PID}}(o_t)
=K_P\(x_t-\sigma\)
+K_I \sum_{\tau=0}^t\(x_{\tau}-\sigma\)
+K_D\frac{\(x_t-\sigma\)-\(x_{t-1}-\sigma\)}{\Delta  t },
\eea
Our model leverages the inductive bias inherent in a PID (Proportional-Integral-Derivative) controller. Specifically, we incorporate tracking errors, integrals, and derivatives as components of the state vector $s_t$. Furthermore, our policy network is designed as a trainable linear framework. This learnable linear framework not only allows for the adjustment of the corresponding $K_P$, $K_I$, and $K_D$ parameters but also enables the extraction of external information, aiding in decision-making from other variables in the state vector. Remarkably, when learned effectively, our policy network can outperform a PID controller, making it a highly adaptable solution.

\paragraph{PPO Model.}
Our methods incorporate the PPO algorithms, EMA reward function, and PID inductive bias. The PPO algorithm is a reinforcement learning algorithm that aims to improve and optimize policy functions for better decision-making in sequential tasks. We choose PPO to optimize our reward function. Instead of calculating reward based on one single spill, we utilize EMA in the reward function to both capture trends in one sequence of spills and reduce the fluctuations. Moreover, we utilize the PID inductive bias in our policy network and state factor. 

